Differentiable Allophone Graphs for Language-Universal Speech Recognition

Building language-universal speech recognition systems entails producing phonological units of spoken sound that can be shared across languages. While speech annotations at the language-specific phoneme or surface levels are readily available, annotations at a universal phone level are relatively rare and difficult to produce. In this work, we present a general framework to derive phone-level supervision from only phonemic transcriptions and phone-to-phoneme mappings with learnable weights represented using weighted finite-state transducers, which we call differentiable allophone graphs. By training multilingually, we build a universal phone-based speech recognition model with interpretable probabilistic phone-to-phoneme mappings for each language. These phone-based systems with learned allophone graphs can be used by linguists to document new languages, build phone-based lexicons that capture rich pronunciation variations, and re-evaluate the allophone mappings of seen language. We demonstrate the aforementioned benefits of our proposed framework with a system trained on 7 diverse languages.

==> tables/masked_phones.tex <==
% \resizebox {\linewidth} {!} {
\begin{tabular}{lcccc}
\toprule
& \multicolumn{2}{c}{Tusom} & \multicolumn{2}{c}{Inuktitut} \\
\cmidrule(r){2-3} \cmidrule(r){4-5}
Model & w/o Mask & w/ Mask & w/o Mask & w/ Mask \\
\midrule
AlloMatrix & 89.1 & 66.1 & 96.7 & - \\
\midrule
AlloGraph & 80.5 & 60.9 & 85.8 & - \\
+ Phone Regularization & 77.7 & \textbf{60.0} & 79.9 & - \\
\bottomrule
\end{tabular}
% }
